ETHcavation: A Dataset and Pipeline for Panoptic Scene Understanding and Object Tracking in Dynamic Construction Environments

Construction sites are challenging environments for autonomous systems due to their unstructured nature and the presence of dynamic actors, such as workers and machinery. This work presents a comprehensive panoptic scene understanding solution designed to handle the complexities of such environments by integrating 2D panoptic segmentation with 3D LiDAR mapping. Our system generates detailed environmental representations in real-time by combining semantic and geometric data, supported by Kalman Filter-based tracking for dynamic object detection. We introduce a fine-tuning method that adapts large pre-trained panoptic segmentation models for construction site applications using a limited number of domain-specific samples. For this use case, we release a first-of-its-kind dataset of 502 hand-labeled sample images with panoptic annotations from construction sites. In addition, we propose a dynamic panoptic mapping technique that enhances scene understanding in unstructured environments. As a case study, we demonstrate the system's application for autonomous navigation, utilizing real-time RRT* for reactive path planning in dynamic scenarios. The dataset (https://leggedrobotics.github.io/panoptic-scene-understanding.github.io/) and code (https://github.com/leggedrobotics/rsl_panoptic_mapping) for training and deployment are publicly available to support future research.

==> _3-ProblemFormulation.tex <==
% Goal: create a panoptic environment representation, extract it, and perform two tasks.
% % Explain the task exactly.
% % "Autonomous planning and navigation."
% Autonomous planning and navigation for construction robots are mostly tackled through geometric information, as described in the last section. The composition of a construction environment is, however, complicated. Thus, the robot requires a deeper understanding and more comprehensive representation of the environment to safely travel from start to goal and interact with its surroundings. In autonomous vehicles, vision-based methods such as image segmentation and object detection are commonly used to provide a semantic representation of the environment. By giving the surroundings semantic meanings, the vehicle is able to identify its targets and make better planning schedules.

% In this work, our goal is to combine the vision-based method with the geometry-based method and create a panoptic environment representation for the construction robot. Furthermore, we extract relevant information from the panoptic representation to autonomously perform two different tasks: navigation and task planning. The panoptic representation provides semantic information for the robot to classify obstacles and traversable ground. Thus the robot can realize path planning and collision checking for autonomous navigation. Moreover, a panoptic representation can provide the location and shape of each instance of a target object. We also employ this instance information for an autonomous stone-grasping task.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}[ht!]
% \centering
% \includegraphics[width=0.95\textwidth]{figures/approach/PipelineOverview2.pdf}
% \caption{Overview of the proposed approach. \textbf{A}: Camera images are fed into the panoptic segmentation network to output panoptic masks. \textbf{B}: The panoptic masks are projected to the according point clouds and the segmented point clouds are aggregated to form a 3D panoptic map. \textbf{C}: Traversability is estimated from the 3D panoptic map. An occupancy map and a semantic cost map are extracted for path planning and collision checking. \textbf{D}: Instances of stones are detected from the panoptic segmentation, and their location and shape are acquired from the panoptic map for the stone grasping task.}
% \label{fig:graph_overview}
% \end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
